Does bilevel optimization result in more competitive racing behavior?

Two-vehicle racing is natural example of a competitive dynamic game. As with most dynamic games, there are many ways in which the underlying solution concept can be structured, resulting in different equilibrium concepts. The assumed solution concept influences the behaviors of two interacting players in racing. For example, blocking behavior emerges naturally in leader-follower play, but to achieve this in Nash play the costs would have to be chosen specifically to trigger this behavior. In this work, we develop a novel model for competitive two-player vehicle racing, represented as an equilibrium problem, complete with simplified aerodynamic drag and drafting effects, as well as position-dependent collision-avoidance responsibility. We use our model to explore how different solution concepts affect competitiveness. We develop a solution for bilevel optimization problems, enabling a large-scale empirical study comparing bilevel strategies (either as leader or follower), Nash equilibrium strategy and a single-player constant velocity baseline. We find the choice of strategies significantly affects competitive performance and safety.

==> game_theory.tex <==
Game theory is the study of interaction of multiple decision-makers, which we will refer to as  \textit{players} or \textit{agents}. It can be viewed as an extension of mathematical programming and optimal control theory. One-player static games are mathematical programming problems, and one-player dynamic games are optimal control problems. Each player's objectives and constraints, without the loss of generality, can be described by a cost function (loss function) and a nonlinear inequality that depends on the player's own and, non-trivially, the others' decision variables. 

We assume that no cooperation is allowed between the players. For simplicity, let us consider a two-player game, where each player has their own strategy represented by the continuous decision variables $x_1\in\mathbb{R}^{n_2}, x_2\in\mathbb{R}^{n_1}$ ($n_1, n_2$ being the number of decision variables), and each player has their own coupled optimization problem ($\mathrm{OP}$s),

\begin{equation}
\begin{aligned}
&\mathrm{OP}_1 \text{ (Player 1)}:\\
&\underset{x_1, x_2}{\min}\quad f_1(x_1, x_2)\\
&\text{s.t}\quad g_1(x_1, x_2) \geq \mathbf{0},
\end{aligned} \hspace{1cm} 
\begin{aligned}
&\mathrm{OP}_2 \text{ (Player 2)}:\\
&\underset{x_1, x_2}{\min}\quad f_2(x_1, x_2)\\
&\text{s.t.}\quad g_2(x_1, x_2) \geq \mathbf{0}. 
\end{aligned}
\label{equation:opts}
\end{equation}
The concept of an optimal strategy that is common to all players is inapplicable in the fully noncooperative setting. For starters, we are interested in feasible strategies that could work for all players, but more importantly we shall seek \textit{equilibrium} strategies that satisfy all players in some sense. Before we can discuss what equilibrium means in this context, we must first talk about the \textit{information structure} of our game. 

It is always possible to consider each optimization problems in isolation, for example we consider $x_2$ as a fixed parameter for $\mathrm{OP}_1$ and $x_1$ as a fixed parameter for $\mathrm{OP}_2$. This would correspond to two independent single-player optimization problems. On the other, we could consider a scheme where the both players make a decision simultaneously and they must reach an equilibrium in the sense no player can gain an advantage by unilaterally modifying their strategy. This corresponds to a flat information structure, where the equilibrium solution must satisfy the Karush–Kuhn–Tucker (KKT) conditions of all players simultaneously. Let us assume $x^* = (x_i, x_{-i})$ is a generalized Nash equilibrium, where subscript $-i$ refers to the strategy of all players except for player $i$, and we note that in the case of two-players $i=\{1,2\}$, then we can define the generalized Nash equilibrium as if it follows for every $i$,

\begin{equation*}
f_i(x_i^*, x_{-i}^*) \leq f_i(x_i, x_{-i}^*),\quad \forall x_i \in X_i,
\end{equation*}
where we can define $X_i = \left\{g_i(x_i, x_{-i}) \geq \mathbf{0}\right\}$ where we consider $g_i:\mathbb{R}^{n_i\times n_{-i}}\rightarrow \mathbb{R}^{m_i}$ for $m_i$ number of constraints. In Nash equilibrium there is no unilateral incentive for any player to unilaterally deviate from their strategy. In the Nash equilibrium information structure, a player cannot reason about how the decisions of other players affect its own objective function. Note that we call it generalized Nash equilibrium because the constraints depend on other player's actions. For the remainder of the paper we will use Nash equilibrium and generalized Nash equilibrium interchangeably.

\begin{figure}[!htb]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
\tikzstyle{block} = [rectangle, draw, %
text width=1cm, text centered, rounded corners, node distance=1.5cm, minimum height=1cm, inner sep=2pt]
\tikzstyle{line} = [draw, -]
\begin{tikzpicture}[auto]
	\node (P1) [block] {$\mathrm{OP}_i$};
	\node (P2) [block, right = of P1] {$\mathrm{OP}_{-i}$};
\end{tikzpicture}
\caption{P1 and P2 in Nash equilibrium}
\end{subfigure}
\vspace{\fill}
\begin{subfigure}[b]{0.2\textwidth}
\centering
\tikzstyle{block} = [rectangle, draw, %
text width=1cm, text centered, rounded corners, node distance=1.5cm, minimum height=1cm, inner sep=2pt]
\tikzstyle{line} = [draw, ->]
\begin{tikzpicture}[auto]
    \node (a) [] {};
	\node (P1) [block, below = .2cm of a] {$\mathrm{OP}_i$};
	\node (P2) [block, below = of P1] {$\mathrm{OP}_{-i}$};
	\path [line] (P1) -- (P2);
\end{tikzpicture}
\caption{P1 as Leader}
\end{subfigure}
\begin{subfigure}[b]{0.2\textwidth}
\centering
\tikzstyle{block} = [rectangle, draw, %
text width=1cm, text centered, rounded corners, node distance=1.5cm, minimum height=1cm, inner sep=2pt]
\tikzstyle{line} = [draw, ->]
\begin{tikzpicture}[auto]
 	\node (P2) [block] {$\mathrm{OP}_2$};
	\node (P1) [block, below = of P2] {$\mathrm{OP}_1$};
    \path [line] (P2) -- (P1);
\end{tikzpicture}
\caption{P2 as Leader}
\end{subfigure}
\caption{Nash equilibrium and bilevel information structure for two players.}
\label{fig:information_structure}
\end{figure}

A natural observation for many two player games is that there exists a hierarchy in the choosing of strategies between the players. If some players can choose their strategies first, and then announce them, we can combine the single-player problems as a bilevel optimization problem. This type of information structure is also referred to as the Stackelberg equilibrium, in the bilevel information structure the player who is the leader solves their problem first, and then the follower must solve their problem based on the leader's strategy. There are two ways to set up the bilevel problem for two players, because we can choose either player as the leader. Let player one be the leader in the two player bilevel game, then the  bilevel problem can be represented as, 

\begin{equation*}
\begin{aligned}
\quad
\underset{x_1}{\min}\quad &f_1(x_1, x_2)\\
\text{s.t.}\quad &g_1(x_1, x_2) \geq \mathbf{0} \\
    &x_2 \text{ solves}\quad \mathrm{OP}_2(x_1, \cdot).
\end{aligned}
\end{equation*}


==> initial_conditions_fig.tex <==

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\captionsetup{width=.9\linewidth}
\includegraphics[width=\columnwidth]{NN_samples.pdf}
\caption{P1 and P2 both choosing strategies by solving for Nash equilibria.}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\captionsetup{width=.9\linewidth}
\includegraphics[width=\columnwidth]{LF_samples.pdf}
\caption{
P1 generates strategies as a leader in bilevel optimization, P2 generates strategies as a follower.
}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\captionsetup{width=.9\linewidth}
\includegraphics[width=\columnwidth]{LL_samples.pdf}
\caption{P1 and P2 both generating strategies by solving a bilevel optimization in which they are the leader.}
\end{subfigure}
\caption{Four different initial conditions in three different competition types for P1 (Blue) and P2 (Red): (a) Nash-Nash competition, (b) Leader-Follower competition, (c) Leader-Leader competition.}
\label{fig:initial_conditions}
\end{figure*}


==> response_to_reviewers.tex <==

We thank our reviewers for their suggestions, please see our responses below:

\section*{Reviewer 1}

\subsection{Limitations}

\begin{enumerate}

\item \textit{The proposed setup only considers a simple scenario with two competitive players moving in a straight lane, taking into account second-order control. The proposed algorithm should be able to adapt to more complex curves, as racing in a straight line is considered less valued.}

\response{We added support for curved tracks, and replaced our simple motion dynamics with a nonlinear simple craft vehicle dynamics model. We updated our description in \cref{subsec:dynamics}.}

\item \textit{The four types of racers represent somewhat of a hard switch with distinct behaviors. In a competitive game, people often care more about when the racer should change their information pattern or leader-follower roles. However, their information currently remains fixed during a race, and, since the two agents are not aware of each other's competition type (even though it could be inferred from their states), the optimization remains passive for now.}

\response{In the beginning of \cref{sec:sim_experiments} we discuss the fixed choice of information pattern. In practice this could change over the course of a simulation run. As you mention, a belief over the information pattern or strategy generation method that an opponent is using could be estimated from previous interaction, and this could be used to solve an imperfect information game, in which one player optimizes against the distribution of strategy generation approaches that the opponent might be using. However, this is beyond the scope of this work. We are attempting to compare the impact of various perfect information, finite-horizon trajectory game models, as are most commonly proposed in the literature.}

\item \textit{The results are intuitive, but I think they still boil down to the prisoner's dilemma, albeit with a different set of descriptions and conditions.}

\response{Great observation! We discuss the emergent higher-level or meta bimatrix game in \cref{subsec:performance} paragraph 3.}

\end{enumerate}

\subsection{Improvements}

\begin{enumerate}

\item \textit{I suggest including a section/subsection for related works, as game-theoretic motion planning might not be a field with which many roboticists are familiar.}

\response{We added a short discussion of some related works in paragraph 6 of \cref{sec:intro}.}

\item \textit{During one player's planning of a $n_T$  horizon, does it have access to the other player's decision? What is the procedure of their decision making?}

\response{We clarify players have access to other player's decisions in \cref{sec:racing_model} paragraph 3.}

\item \textit{The metric "mean simulation step" can only reflect the safety of the game. For a competitive game, I suggest using some metrics (e.g. elo rating, TrueSkill) to quantify the performance of each type of players.}

\response{We use total cost because we want the competition metric to reflect the cost that the players are actually optimizing for. Other metrics such as time to finish would not be directly considered in the players' optimization problems.}

\item \textit{It would be nice to discuss the complexity of computing the bilevel equilibria since it is more of a theoretical study.}

\response{We discuss complexity of computing bilevel equilibria at the end of \cref{sec:bilevel}.}

\item \textit{Since the solver can get stuck in some local equilibrium points or fail to find an equilibrium, does the/a Nash equilibrium always exist in this general racing game?}

\response{We explain existence of Nash equilibria at the end of \cref{sec:nash}.}

\end{enumerate}

\subsection{Clarity}

\begin{enumerate}

\item \textit{The vector $0$  should be consistently styled in either regular or boldface.} 

\response{Fixed, thank you.}

\item \textit{In section VI.B, regarding cost functions, there seems to be a mix-up between the state $y$ and position $p$.}

\response{We made sure the cost and constraint function uses $p_i$ consistently to refer to $i$\textsuperscript{th} player position.}

\item \textit{I suppose $c_d$ to be a drag/dumping coefficient? This is not mentioned.}

\response{We renamed $c_d$ to $c_\text{drag}$ and referred to it in \cref{subsec:dynamics} paragraph 2.}

\end{enumerate}

\section*{Reviewer 2}

\subsection{Limitations}

\begin{enumerate}

\item \textit{The paper suffers from a relative lack of theoretical novelty, as it leverages, standard formulations and approaches. }

\response{We do not necessarily claim that we present a novel method which results in state-of-the-art racing behavior. Any such result would be environment and platform-dependent, and while our model has many advanced and realistic components (drafting effects, aerodynamic drag, and in the new version, non-linear vehicle dynamics, curved tracks), it is still a relatively simple model.}

\response{Rather, the novelty of our work is in the systematic analysis of the advantage posed by different choice of information pattern when solving games in a model-predictive-gameplay manner. We use our racing model as a sufficiently rich vessel to study this problem. As far as we know, no other work has performed such an analysis. Another important novel component of this work is in using a proper bilevel solver to compute leader-follower equilibria. Previous works (that we are aware of) that postulated that hierarchical interactions might result in more strategic behavior did not ever actually solve for Stackelberg equilibrium points. Rather, they used heuristic approaches to approximate Stackelberg equilibria.}

\response{We do not believe that solving constrained, non-convex bilevel optimization problems is standard, as you say. That is true for solving any form of game with constraints and non-trivial information pattern. There do not exist open-source bilevel solvers which can be used off-the-shelf to solve the problems we study in this work. This is why previous works used heuristic approaches, and why we chose to implement a proper solver for the purpose of this work (and have made it available on our project github repository). We tried to clarify the novel aspect of our work in \cref{sec:intro}}.

\item \textit{The statistical relevance of the results does not appear to be extremely strong, furthermore, it is a bit counterintuitive to pit against leader vs leader and follower vs follower, i.e. assuming partial information, in methods that are developed for perfect information games.}

\response{We discuss statistical significance in \cref{subsec:performance}. As stated in response to the previous point, our work is not necessarily claiming that we have invented a novel procedure for producing better racing behavior. Rather, we are claiming that when solving for proper Stackelberg equilibria, there is a marginal improvement over other comparable approaches (like solving for Nash equilibria or using constant-velocity MPC), but that Stackelberg equilibria alone are not enough to generate some behaviors (like blocking) that might previously be associated with bilevel formulations.}

\response{Furthermore, we attempted to clarify and address your comments about pitting equilibria from perfect-information games like leader vs. leader in the first few paragraphs of \cref{sec:sim_experiments}. In essence, while solving for equilibrium points in an imperfect information model (and even better, one which models repeated interaction) would be ideal, such formulations are much more complicated to solve. It is commonly suggested in other works to e.g. use Nash equilibrium strategies in a model-predictive gameplay in contexts such as a self-driving car interacting with humans. However, that also is a partial information setting, and while solving a finite-horizon static/open-loop Nash equilibrium problem is not an exact model, it is still a valid and useful technique for generating interaction-aware strategies. We believe that studying the implications of different choices (other than static Nash) of finite-horizon perfect information games, to be used in such settings, is a valid and important pursuit. }

\item \textit{The realism and applicability of the dynamics to real-world ground vehicles are also limited.}

\response{We replaced simple motion with nonlinear simple craft dynamics, and curved roads for increased realism and applicability of the dynamics.}

\end{enumerate}

\subsection{Improvements}

\begin{enumerate}

\item \textit{"This purpose of this study" (sic)}

\response{Fixed, thank you.}

\item \textit{The velocity penalty is stated to be the "most" competitive part of the cost function, how do the other components encourage competition?}

\response{We corrected and clarified that the third component of the cost function is the only competitive component of the cost in \cref{subsec:obj_func} paragraph 2.}

\item \textit{What is the role of responsibility in the optimization problem?}

\response{We clarify in \cref{sec:responsibility} that the technique we introduce for collision-avoidance responsibility does not fundamentally change the nature of the game being solved from existence/computation perspectives. Standard collision-avoidance constraints already depend on the strategies of the other players, resulting in "generalized" equilibrium problems. When using the strategy-dependent modifications to induce "responsibility", we are just choosing a different form of generalized constraint.}

\item \textit{ What is the formalization of the optimization problem for the single-player strategy?}

\response{We clarify the single-player optimization problem in \cref{sec:sim_experiments} paragraph 1}

\item \textit{In the caption of table III, "inevitable constraint violation", what does inevitable mean here?}

\response{We have reworded the caption for clarity.}

\end{enumerate}

\section*{Reviewer 3}

\subsection{Limitations}

\begin{enumerate}

\item \textit{The fit of the paper to RSS is not clear. While game theory is certainly relevant to robotic decision-making, the paper doesn't position itself to clearly address this community, either through motivating examples or via demonstration in a robotics test domain. The paper feels more appropriate to an AI or Agents conference. To put plainly: what impact does this result have on how we solve robotic decision-making problems, what could/should a roboticist do with this result?}

\response{We added motivating examples in paragraph 5 of \cref{sec:intro}}

\item \textit{The presentation of the results is at time difficult to understand. For example}

\response{We agree.}

\item \textit{Fig. 3 is hard to interpret and I'm not sure I see how it connects with what's described in the caption.}

\response{We agree that Fig. 3 was hard to interpret. We decided to remove previously Fig. 3 and Fig. 4 in lieu of more tables and discussion of our updated simulation results using the new nonlinear dynamics and curved tracks, more reasons for their removal explained below.}

\item \textit{The large dip in Fig. 4 is never explained. Also, why not include the results for the single-player competition here or in Fig. 5?}

\response{We hypothesize the large dip in Fig. 4 was probably a spurious correlation in the way we were initializing the players that gave an unintended advantage to the ego player. We did not observe the dip for our updated simulation results. We chose not to include the results for the other competitions in order to avoid overcrowding then Fig 4. Other motivations for removal of Fig. 3 and Fig. 4 is avoiding the unintended emphasis on the N-N vs. L-F comparison, we should be comparing all information patterns, and after adding all reviewer suggestions the length of the paper has grown substantially.}

\item \textit{Why are the numbers in Table IV not symmetric?}

\response{Table IV used to contain 
We have clarified Table IV by splitting it into two parts}

\end{enumerate}

\subsection{Improvements}

\begin{enumerate}

\item \textit{"different combination of" \textrightarrow  "different combinations of"}

\response{Fixed, thank you.}

\item \textit{"continuous, twice differentiable cost function" is this a requirement of the optimisation?}

\response{We clarify that this is a requirement for our method in \cref{sec:game_theory}, paragraph 2.}

\item \textit{"necessary but sufficient" \textrightarrow  "necessary but insufficient" or "necessary and sufficient"?}

\response{Fixed, should be "necessary but not sufficient"}
    
\item \textit{"at every simulation step, and every simulation step" repetition unnecessary}

\response{Fixed, thank you.}
    
\item \textit{"be to the vehicle state" \textrightarrow  "be the vehicle state"}

\response{Fixed, thank you.}

\item \textit{"SP" is not explicitly defined in the text as "single-player"}

\response{Clarified in the beginning of \cref{sec:sim_experiments}.}

\item \textit{ In table III, are these number of "steps" before constraint violation or number of "runs"? If the latter, what does a "run" constitute?}

\response{Clarified caption.}

\item \textit{"safe choice to assume for the players to assume"  \textrightarrow "safe choice for the players to assume"}

\response{Fixed, thank you.}

\item \textit{"if the both players" \textrightarrow "if both players"}
    
\response{Fixed, thank you.}

\end{enumerate}



==> simulations.tex <==

\begin{figure*}[!htb]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\columnwidth]{mode3.png}
\caption{P1 and P2 has agreed to the Nash competition.}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\columnwidth]{mode9.png}
\caption{P1 and P2 has agreed to the bilevel competition, and that P1 is the leader.}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\columnwidth]{mode6.png}
\caption{P1 and P2 has agreed to the  bilevel competition, but they incorrectly believe they are both the leader.}
\end{subfigure}
\caption{Four different initial conditions in three different competition types for P1 (Blue) and P2 (Red): (a) Nash competition, (b) bilevel competition, (c) bilevel competition with disagreement. When the players do not agree on the competition type as in sub-figure (c), we superimposed the opponent's contradictory plan with transparency.}
\label{fig:initial_conditions}
\end{figure*}

In this section we compare 16 different competition types as a combination of different information patterns using our two-player racing model that was detailed in \cref{sec:racing_model} using a large scale randomized simulation trial. In the distributed brain scenario, where the players do not have to agree on the information structure, each player can unilaterally choose from one of the four information patterns, without knowing what the other player will do. We enumerate the 16 different competition types that we investigate in this study in \cref{tab:competition_types}. In \cref{tab:competition_types} and the other tables that follow it, the columns represent Player 1's assumed equilibrium type, while the rows represent Player 2's assumed equilibrium type. We use ``S, N, L, F'' as a shorthand to single-player (SP), Nash, Leader and Follower to refer to the information pattern assumed by the players.

\begin{table}[!htb]
\centering
\caption{Competition types.}
	\begin{tabular}{rllll}
	\toprule
	  \diagbox{P2}{P1} & SP (S) & Nash (N) & Leader (L) & Follower (F)\\
	\midrule
	SP (S) & S-S &  N-S & L-S &  F-S \\
	Nash (N) & S-N & N-N  &  L-N & F-N  \\
 	Leader (L)& S-L & N-L & L-L  &  F-L \\
 Follower (F) & S-F &  N-F & L-F &  F-F \\
 	\bottomrule
	\end{tabular}
\label{tab:competition_types}
\end{table}

Due to the symmetry in the information patterns, we only have to compute 10 different competition types for each initial condition in order to fill this table, which we arbitrarily chose as the lower-triangular section of \cref{tab:competition_types}, including the diagonal. 

For each competition type we have simulated 2000 randomly generated feasible initial conditions for 50 time steps, using $n_T=10$ number computation horizon time steps. The other parameters of our model and simulation are listed in \cref{tab:sim_params}  When we generated the random initial conditions, we first chose the first player's lateral position from a uniform distribution between the lateral road limits. Then, the second player's position was chosen from a uniform radial distribution of minimum and maximum radius based on the desired minimum collision radius, and if necessary it was resampled to remain within the lateral road limits. Then for the initial velocities, the first player's longitudinal velocity is sampled from a uniform non-negative range, while the second player's longitudinal velocity is computed as a uniformly distributed offset compared to the first player's velocity. The initial lateral velocities were kept at zero. 

We showcase a small sample of initial conditions and the first time step motion plans that correspond to different competition types in \cref{fig:initial_conditions}. In \cref{fig:initial_conditions} (c), we overlay the realized simulation and the mistaken expectations of the players, where the transparent plans correspond to each player's incorrect expectation that the opponent will play as a follower, e.g.  the transparent Red trajectory is what Blue thinks Red would do as a follower, and vice versa.

\begin{table}[!htb]
\centering
\caption{Simulation and game parameters.}
	\begin{tabular}{rS[table-omit-exponent]|rS}
	\toprule
    Parameter & {Value} & Parameter & {Value}\\
	\midrule
	$\alpha_1$ & 1e-3  &  $u_\text{max} ^\text{nom}$ & \qty{1.0}{\meter\second^{-2}} \\
    $\alpha_2$ &  1e-4 & $u_\text{max}^\text{brake}$ &  \qty{5.0}{\meter\second^{-2}}\\
    $\beta$ & 1e-1 & $u_\text{max}^\text{draft}$& \qty{2.5}{\meter\second^{-2}} \\
    $n_T$ & 10 &$y_\text{min}^\text{lat}$  & \qty{-2.}{\meter}\\
    $\Delta t$ & \qty{1e-1}{\second}& $y_\text{max}^\text{lat}$& \qty{2.}{\meter} \\
    $r_\text{desired}$ & \qty{1.2}{\meter} &$\dot{y}_{1,0, \text{min}}^\text{long}$ & \qty{1.5}{\meter\second^{-1}}  \\
    $c_d$ &\qty{.2}{\second^{-1}} & $\dot{y}_{1,0, \text{max}}^\text{long}$ & \qty{3.0}{\meter\second^{-1}}\\
    $r$ & \qty{1.0}{\meter} & $\dot{y}_{2,0, \Delta}^\text{long}$ & \qty{1.5}{\meter\second^{-1}}\\
      $\ell_\text{draft}$ & \qty{5.0}{\meter} & $w_\text{draft}$ & \qty{2.0}{\meter} \\
 	\bottomrule
	\end{tabular}
\label{tab:sim_params}
\end{table}


Solving bilevel problems poses a significant challenge due to their sensitivity to initialization of the solver. Depending on the initialization, the solver can get stuck in a disadvantageous local equilibrium points or fail to find an equilibrium. Because of this, we follow a fallback strategy when we are solving for the bilevel equilibrium. We initialize the bilevel solver using the Nash equilibrium solution, in the event that the solver fails to reach an equilibrium, we fall back to using the single-player solution as our initialization. 
In the case this all fails, we fall back to an uncontrolled simulation step in the hopes that the situation may improve in the subsequent iterations. Most importantly, at the start of every simulation step, we manually check all constraints. If the initial position and velocities of the players violate the constraints such as the lateral road limits or the spatial collision constraints, we terminate the simulation on the basis of safety constraint violation.

\subsection{Robustness}

Our metric for robustness is the mean number of steps of the simulation before the simulation is terminated due to one of the safety constraint violation scenarios: (i) One of the players was forced out of the road, or (ii) the players found themselves in an unavoidable player-to-player collision. We compile the results in \cref{tab:steps} for all competition types.

Our results indicate that there is no significant difference in safety between the baseline single-player and Nash equilibrium competitions. However, this is not true for the bilevel competition. Playing as a leader causes increased competitive behavior on the part of the ego player, however this increased aggression is reflected as decreased safety. On the other hand, we observe that playing as a follower leads to decreased aggression and therefore increased safety. Independent of what the opponent does, the most dangerous strategy for the ego player is to assume that they are the leader. Similarly, the safest strategy for the ego player is to assume that they are the follower.

\begin{table}[!htb]
\centering
\caption{Mean number of simulation steps before a safety constraint violation for different competition types  ($\pm$95\% CI)}
	\begin{tabular}{
     r
     S[table-format=2.1(1), separate-uncertainty]
     S[table-format=2.1(1), separate-uncertainty]
     S[table-format=2.1(1), separate-uncertainty]
     S[table-format=2.1(1), separate-uncertainty]
     }
	\toprule
	\diagbox{P2}{P1} & {SP (S)} & {Nash (N)} & {Leader (L)} & {Follower (F)} \\
	\midrule
	SP (S) & 45.0(5) & 39.6(6) & 30.8(7) & 42.1(6)  \\
	Nash (N)& 39.6(6) & 39.8(6) & 29.4(7) &44.3(5) \\
    Leader (L) & 30.8(7) & 29.4(7) & 21.0(6) & 34.5(7) \\
    Follower (F) & 42.1(6) & 44.3(5) & 34.5(7) & 47.5(4) \\
    \midrule
    Average & 39.4(3) & 38.3(4) & 28.9(5) & 42.1(3) \\
 	\bottomrule
	\end{tabular}
\label{tab:steps}
\end{table}

We observe that the leader-leader competition leads to the lowest mean number of simulation steps before termination. We stipulate this is due to the players having a false sense of confidence about their ability to enforce their strategies on their opponent. This situation naturally leads to increased rates of collision, and the worst case scenario occurs when both players incorrectly believe that they are the leader in a bilevel game. Furthermore, the Follower-Follower scenario scores highest in terms of mean time steps before safety constraint violation. In this section we have shown that the mean number of simulation steps before a safety violation depends significantly on the competition type.

\subsection{Performance}

In this section we compare the performance of different competition types and we use the mean running cost as our metric for competitive advantage. In \cref {fig:running_cost}, we plot the average cost per time step for Nash and bilevel competition information patterns with respect to simulation steps. We observe that the most competitive behavior occurs at the beginning of the simulation, and most of the interaction concludes after about 20 simulation steps. We display the statistical distribution of mean running cost per step for the Nash and bilevel competitions in \cref {fig:box_plot}, which corresponds to each line in \cref {fig:running_cost}. Unsurprisingly, single-player and Nash competition leads to an average cost of zero within the confidence limit, while the bilevel competition leads to decreased cost for the ego player who is playing as the leader.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{plot_3_v_9_running_cost.pdf}
\caption{Mean running costs for the ego player when both players agree on Nash equilibrium (N-N) or bilevel (L-F) competition type with respect to all initial conditions and time steps. The shaded area is the 95\% confidence interval.}
\label{fig:running_cost}
\end{figure}

 
\begin{figure}[]
\centering
\includegraphics[width=0.9\columnwidth]{boxplot_running_cost.pdf}
\caption{Mean running cost compared with respect to different competition types. (Whiskers of the box plot corresponds to the $1.5\mathrm{IQR}$.)}
\label{fig:box_plot}
\end{figure}

\begin{table}[!htb]
\centering
\caption{Mean running costs of different combinations of competition types for the ego player, P1 ($\pm$95\% CI).}
	\begin{tabular}{
     r
     S[table-format=2.2(2), separate-uncertainty]
     S[table-format=2.2(2), separate-uncertainty]
     S[table-format=2.2(2), separate-uncertainty]
     S[table-format=2.2(2), separate-uncertainty]
     }
	\toprule
	$10^{-3}$ & {S} & {N} & {L} & {F} \\
	\midrule
	S & 1.75(122) & 0.83(143) & -11.50 (22) & 7.84(128)  \\
	N &  0.82(14) & 0.24(147) & -8.06(206) & 9.38(115) \\
 	L & 13.50(23) & 10.20(21) & 1.24 (254) &  17.30(18) \\
    F & -6.33(128) & -7.88(114) & -15.40(18) & 0.92(90) \\
    \midrule
    Avg. & 2.43(127) & 0.85(76) & -8.42(88) & 8.86(76) \\
 	\bottomrule
	\end{tabular}
\label{tab:total_costs}
\end{table}

We compile the performance of the ego player for different competition types in \cref{tab:total_costs}. If both players that agree Nash competition, there is no competitive advantage to be exploited by either player, and the baseline single-player results are similar to the Nash competition. On the other hand, bilevel competition leads  Playing leader against an opponent that plays follower provides the best competitive advantage, while the difference between playing single-player and Nash equilibrium is negligible. The values are not symmetric with respect to the diagonal because the total cost includes center of lane and control components, and is not zero-sum.

We observe that the bilevel competition leads to increased competitive advantage to the leader, which is reflected as disadvantage to the follower. Assuming to play as the follower comes at a cost penalty even against an opponent who is thinks the game that is played in single-player or Nash competition. The competitive advantage comes with increased collision risk and therefore reduced safety as we have discussed in the previous section, especially if both players greedily assume that they are the leader, the likelihood of a collision or road limit violation increases significantly. On the other hand, it is always a safe choice for the players to unilaterally assume that they are the follower, but it can be exploited by a risk-taking opponent that unilaterally assumes to be the leader. 
We observe that the bilevel competition leads to increased competitive advantage to the leader, which is reflected as disadvantage to the follower. Assuming to play as the follower comes at a cost penalty even against an opponent who is thinks the game that is played in single-player or Nash competition. The competitive advantage comes with increased collision risk and therefore reduced safety as we have discussed in the previous section, especially if both players greedily assume that they are the leader, the likelihood of a collision or road limit violation increases significantly. On the other hand, it is always a safe choice for the players to unilaterally assume that they are the follower, but it can be exploited by a risk-taking opponent that unilaterally assumes to be the leader. 

